AUFormer: Vision Transformers are Parameter-Efficient Facial Action Unit Detectors

Facial Action Units (AU) is a vital concept in the realm of affective computing, and AU detection has always been a hot research topic. Existing methods suffer from overfitting issues due to the utilization of a large number of learnable parameters on scarce AU-annotated datasets or heavy reliance on substantial additional relevant data. Parameter-Efficient Transfer Learning (PETL) provides a promising paradigm to address these challenges, whereas its existing methods lack design for AU characteristics. Therefore, we innovatively investigate PETL paradigm to AU detection, introducing AUFormer and proposing a novel Mixture-of-Knowledge Expert (MoKE) collaboration mechanism. An individual MoKE specific to a certain AU with minimal learnable parameters first integrates personalized multi-scale and correlation knowledge. Then the MoKE collaborates with other MoKEs in the expert group to obtain aggregated information and inject it into the frozen Vision Transformer (ViT) to achieve parameter-efficient AU detection. Additionally, we design a Margin-truncated Difficulty-aware Weighted Asymmetric Loss (MDWA-Loss), which can encourage the model to focus more on activated AUs, differentiate the difficulty of unactivated AUs, and discard potential mislabeled samples. Extensive experiments from various perspectives, including within-domain, cross-domain, data efficiency, and micro-expression domain, demonstrate AUFormer's state-of-the-art performance and robust generalization abilities without relying on additional relevant data. The code for AUFormer is available at https://github.com/yuankaishen2001/AUFormer.

==> Fig_Tab/BP4D.tex <==
\begin{table*}[t]
\centering
\footnotesize
\caption{F1-score (in \%) for 12 AUs on BP4D. The best and second best results for each column are bolded and underlined, respectively.}
\label{tab:BP4D}
\begin{tabular}{>{\raggedright\arraybackslash}p{2.2cm} | >{\centering\arraybackslash}p{1.3cm} | >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} | >{\centering\arraybackslash}p{0.55cm}}
\toprule[1pt]
\multirow{2}{*}{Method} & \multirow{2}{*}{Venue} & \multicolumn{12}{c|}{AU} & \multirow{2}{*}{\textbf{Avg.}} \\
\cmidrule(lr){3-14}
~ & ~ & 1 & 2 & 4 & 6 & 7 & 10 & 12 & 14 & 15 & 17 & 23 & 24 & ~ \\
\midrule
DRML~\cite{DRML} & CVPR 16 & 36.4 & 41.8 & 43.0 & 55.0 & 67.0 & 66.3 & 65.8 & 54.1 & 33.2 & 48.0 & 31.7 & 30.0 & 48.3 \\

LP-Net~\cite{LP-Net} & CVPR 19 & 43.4 & 38.0 & 54.2 & 77.1 & 76.7 & 83.8 & 87.2 & 63.3 & 45.3 & 60.5 & 48.1 & 54.2 & 61.0 \\

SRERL~\cite{SRERL} & AAAI 19 & 46.9 & 45.3 & 55.6 & 77.1 & 78.4 & 83.5 & 87.6 & 63.9 & 52.2 & 63.9 & 47.1 & 53.3 & 62.9 \\

J{\^A}A-Net~\cite{JAA-Net} & IJCV 21 & 53.8 & 47.8 & 58.2 & 78.5 & 75.8 & 82.7 & 88.2 & 63.7 & 43.3 & 61.8 & 45.6 & 49.9 & 62.4 \\

HMP-PS~\cite{HMP-PS} & CVPR 21 & 53.1 & 46.1 & 56.0 & 76.5 & 76.9 & 82.1 & 86.4 & 64.8 & 51.5 & 63.0 & 49.9 & 54.5 & 63.4 \\

SEV-Net~\cite{SEV-Net} & CVPR 21 & \textbf{58.2} & 50.4 & 58.3 & \textbf{81.9} & 73.9 & \textbf{87.8} & 87.5 & 61.6 & 52.6 & 62.2 & 44.6 & 47.6 & 63.9 \\

FAUDT~\cite{FAUDT} & CVPR 21 & 51.7 & 49.3 & 61.0 & 77.8 & 79.5 & 82.9 & 86.3 & 67.6 & 51.9 & 63.0 & 43.7 & \underline{56.3} & 64.2 \\

PIAP~\cite{PIAP} & ICCV 21 & 54.2 & 47.1 & 54.0 & 79.0 & 78.2 & \underline{86.3} & \textbf{89.5} & 66.1 & 49.7 & 63.2 & 49.9 & 52.0 & 64.1 \\

KDSRL~\cite{KDSRL} & CVPR 22 & 53.3 & 47.4 & 56.2 & 79.4 & 80.7 & 85.1 & 89.0 & 67.4 & \textbf{55.9} & 61.9 & 48.5 & 49.0 & 64.5 \\

ME-GraphAU~\cite{ME-GraphAU} & IJCAI 22 & 52.7 & 44.3 & 60.9 & \underline{79.9} & 80.1 & 85.3 & 89.2 & \textbf{69.4} & \underline{55.4} & 64.4 & 49.8 & 55.1 & \underline{65.5} \\ 

BG-AU~\cite{BG-AU} & CVPR 23 & \underline{57.4} & \textbf{52.6} & \textbf{64.6} & 79.3 & \underline{81.5} & 82.7 & 85.6 & 67.9 & 47.3 & 58.0 & 47.0 & 44.9 & 64.1 \\

KS~\cite{KS} & ICCV 23 & 55.3 & 48.6 & 57.1 & 77.5 & \textbf{81.8} & 83.3 & 86.4 & 62.8 & 52.3 & 61.3 & \textbf{51.6} & \textbf{58.3} & 64.7 \\

FG-Net~\cite{FG-Net} & WACV 24 & 52.6 & 48.8 & 57.1 & 79.8 & 77.5 & 85.6 & \underline{89.3} & \underline{68.0} & 45.6 & \underline{64.8} & 46.2 & 55.7 & 64.3 \\


\midrule

\rowcolor{gray!30}
\textbf{AUFormer (Ours)} & - & 55.2 & \underline{52.2} & \underline{63.2} & 79.3 & 79.7 & 84.2 & 88.6 & 67.0 & 53.3 & \textbf{65.5} & \underline{50.6} & 55.7 & \textbf{66.2} \\


\bottomrule[1pt]
\end{tabular}
\end{table*}

==> Fig_Tab/CAM.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/CAM.pdf}
    \vspace{-1.0em}
    \caption{
    Activation maps for MoKEs corresponding to activated AUs generated using Grad-CAM.
    }
    \label{CAM}
    \vspace{-2.0em}
\end{figure}

==> Fig_Tab/DISFA.tex <==
\begin{table*}[t]
\centering
\footnotesize
\caption{F1-score (in \%) for 8 AUs on DISFA. The best and second best results for each column are bolded and underlined, respectively.}
\label{tab:DISFA}
\begin{tabular}{>{\raggedright\arraybackslash}p{2.2cm} | >{\centering\arraybackslash}p{1.3cm} | >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm} >{\centering\arraybackslash}p{0.5cm}|  >{\centering\arraybackslash}p{0.55cm}}

\toprule[1pt]

\multirow{2}{*}{Method} & \multirow{2}{*}{Venue} & \multicolumn{8}{c|}{AU} & \multirow{2}{*}{\textbf{Avg.}} \\
\cmidrule(lr){3-10}
~ & ~ & 1 & 2 & 4 & 6 & 9 & 12 & 25 & 26 & ~ \\
\midrule

DRML~\cite{DRML} & CVPR 16 & 17.3 & 17.7 & 37.4 & 29.0 & 10.7 & 37.7 & 38.5 & 20.1 & 26.7 \\ 

LP-Net~\cite{LP-Net} & CVPR 19 & 29.9 & 24.7 & 72.7 & 46.8 & 49.6 & 72.9 & 93.8 & 65.0 & 56.9 \\ 

SRERL~\cite{SRERL} & AAAI 19 & 45.7 & 47.8 & 59.6 & 47.1 & 45.6 & 73.5 & 84.3 & 43.6 & 55.9 \\ 

J{\^A}A-Net~\cite{JAA-Net} & IJCV 21 & \underline{62.4} & 60.7 & 67.1 & 41.1 & 45.1 & 73.5 & 90.9 & \underline{67.4} & 63.5 \\

HMP-PS~\cite{HMP-PS} & CVPR 21 & 38.0 & 45.9 & 65.2 & 50.9 & 50.8 & 76.0 & 93.3 & \textbf{67.6} & 61.0 \\

SEV-Net~\cite{SEV-Net} & CVPR 21 & 55.3 & 53.1 & 61.5 & 53.6 & 38.2 & 71.6 & \textbf{95.7} & 41.5 & 58.8 \\

FAUDT~\cite{FAUDT} & CVPR 21 & 46.1 & 48.6 & \underline{72.8} & \textbf{56.7} & 50.0 & 72.1 & 90.8 & 55.4 & 61.5 \\ 

PIAP~\cite{PIAP} & ICCV 21 & 50.2 & 51.8 & 71.9 & 50.6 & \underline{54.5} & \textbf{79.7} & \underline{94.1} & 57.2 & 63.8 \\

KDSRL~\cite{KDSRL} & CVPR 22 & 60.4 & 59.2 & 67.5 & 52.7 & 51.5 & 76.1 & 91.3 & 57.7 & 64.5 \\

ME-GraphAU~\cite{ME-GraphAU} & IJCAI 22 & 52.5 & 45.7 & \textbf{76.1} & 51.8 & 46.5 & 76.1 & 92.9 & 57.6 & 62.4 \\ 

BG-AU~\cite{BG-AU} & CVPR 23 & 41.5 & 44.9 & 60.3 & 51.5 & 50.3 & 70.4 & 91.3 & 55.3 & 58.2 \\

KS~\cite{KS} & ICCV 23 & 53.8 & 59.9 & 69.2 & \underline{54.2} & 50.8 & 75.8 & 92.2 & 46.8 & 62.8 \\

FG-Net~\cite{FG-Net} & WACV 24 & \textbf{63.6} & \textbf{66.9} & 72.5 & 50.7 & 48.8 & \underline{76.5} & \underline{94.1} & 50.1 & \underline{65.4} \\


\midrule

\rowcolor{gray!30}
\textbf{AUFormer (Ours)} & - & 58.6 & \underline{61.0} & 70.4 & 52.4 & \textbf{58.1} & 73.0 & 90.8 & 66.9 & \textbf{66.4} \\

\bottomrule[1pt]
\end{tabular}
\end{table*}

==> Fig_Tab/Hyperparameter.tex <==
% overall table of all ablations
\begin{table*}[t]
\vspace{-.2em}
\centering
\caption{The average F1-score results (in \%) on BP4D with different parameter or setting choices. Default settings are marked in \colorbox{baselinecolor}{gray}.}
\vspace{-.5em}
\label{tab:ablations}
%#################################################
% Type of Adaptation Modules
%#################################################
\subfloat[
Type of adaptation modules.
\label{tab:TypeOfAdaptationModule}
]{
\centering
\begin{minipage}{0.21\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{35}|x{25}}
\toprule[1pt]
Type & Avg. \\
\midrule
Adapter & 63.1  \\
LoRA & 63.0 \\
VPT & 62.6  \\
\rowcolor{gray!30}
Convpass & \textbf{63.6}  \\
\bottomrule[1pt]
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
% Placement of Convpass
%#################################################
\subfloat[
Placement of Convpass.
\label{tab:PlacementOfConvpass}
]{
\begin{minipage}{0.21\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{50}|x{25}}
\toprule[1pt]
Placement & Avg. \\
\midrule
MHSA & 63.0  \\
MLP & 62.9  \\
\rowcolor{gray!30}
MHSA \& MLP & \textbf{63.6}  \\
\bottomrule[1pt]
\multicolumn{2}{c}{~}\\

\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
% Reduced Channel Numbers
%#################################################
\subfloat[
Reduced channel numbers $d$.
\label{tab:ReducedChannelNumbers}
]{
\begin{minipage}{0.21\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{25}|x{25}}
\toprule[1pt]
$d$ & Avg. \\
\midrule
\rowcolor{gray!30}
4 & \textbf{66.2} \\
8 & 65.8 \\
16 & 65.5 \\
32 & 65.4 \\
\bottomrule[1pt]
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
% Dilation Rate in MRF.
%#################################################
\subfloat[
Dilation rate in MRF.
\label{tab:DilationRateInMRF}
]{
\begin{minipage}{0.21\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{54}|x{25}}
\toprule[1pt]
Delation rate & Avg. \\
\midrule
\rowcolor{gray!30}
1, 3, 5 & \textbf{66.2}  \\
1, 3 & 65.8  \\
1 & 65.5  \\
1, 2, 3 & 65.8  \\

\bottomrule[1pt]
\end{tabular}
\end{center}}\end{minipage}
}
\\
\centering
\vspace{0.5em}
%#################################################
% Type of Correlation Matrix in CA
%#################################################
\subfloat[
Calculation method for the correlation matrices in CA.
\label{tab:CalculationMethodInCA}
]{
\begin{minipage}{0.21\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{40}|x{25}}
\toprule[1pt]
Method & Avg. \\
\midrule
Addition & 65.7 \\
Subtraction & 65.6 \\
\rowcolor{gray!30}
Hadamard & \textbf{66.2} \\
\bottomrule[1pt]
\multicolumn{2}{c}{~}\\

\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
% Size of the correlation neighborhood in CA.
%#################################################
\subfloat[
Size of the correlation neighborhood in CA.
\label{tab:CorrelationNeighborhoodInCA}
]{
\begin{minipage}{0.21\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{50}|x{25}}
\toprule[1pt]
Size & Avg. \\
\midrule
\rowcolor{gray!30}
$3 \times 3$ & \textbf{66.2} \\
$5 \times 5$ & 65.8 \\
$7 \times 7$ & 65.9 \\
\bottomrule[1pt]
\multicolumn{2}{c}{~}\\
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
\subfloat[
Left and right boundaries $L$ and $R$ of $\gamma$ in MDWA-Loss.
\label{tab:GammaBoundaries}
]{
\begin{minipage}{0.21\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{60}|x{25}}
\toprule[1pt]
Boundaries of $\gamma$ & Avg. \\
\midrule
$L = R = 1$ & 65.1 \\
$L = 1, R = 1.5$ & 65.1 \\
\rowcolor{gray!30}
$L = 1, R = 2$ & \textbf{65.6} \\
$L = 1.5, R = 2$ & 65.2 \\
\bottomrule[1pt]
\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
\subfloat[
Truncation margin $m$ in MDWA-Loss.
\label{tab:TruncatedMargin}
]{
\begin{minipage}{0.21\linewidth}{\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{45}|x{25}}
\toprule[1pt]
$m$ & Avg. \\
\midrule
0.01 & 65.6\\
0.05 & 65.9 \\
\rowcolor{gray!30}
0.1 & \textbf{66.2} \\
0.2 & 65.4 \\
\bottomrule[1pt]
\end{tabular}
\end{center}}\end{minipage}
}
\vspace{-.5em}
\end{table*}
%##################################################################################################

==> Fig_Tab/Hyperparameter_2.tex <==
\begin{table}[t]
\scriptsize
\centering
\caption{The average F1-score (in \%) on BP4D with different parameter or setting choices. Default settings are marked in \colorbox{baselinecolor}{gray}.}
\vspace{-1.2em}
\label{tab:hyperparameter_2}
%#################################################
% Placement of Convpass
%#################################################
\subfloat[
Placement of Convpass.
\label{tab:PlacementOfConvpass}
]{
\begin{minipage}{0.45\linewidth}{\begin{center}
% \tablestyle{4pt}{1.05}
\begin{tabular}{x{55}|x{25}}
\toprule[1pt]
Placement & Avg. \\
\midrule
MHSA & 63.0  \\
MLP & 62.9  \\
\rowcolor{gray!30}
MHSA \& MLP & \textbf{63.6}  \\
\bottomrule[1pt]
\multicolumn{2}{c}{~}\\

\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
% Reduced Channel Numbers
%#################################################
\subfloat[
Reduced channel numbers $d$.
\label{tab:ReducedChannelNumbers}
]{
\begin{minipage}{0.45\linewidth}{\begin{center}
% \tablestyle{4pt}{1.05}
\begin{tabular}{x{35}|x{25}}
\toprule[1pt]
$d$ & Avg. \\
\midrule
\rowcolor{gray!30}
4 & \textbf{66.2} \\
8 & 65.8 \\
16 & 65.5 \\
32 & 65.4 \\
\bottomrule[1pt]
\end{tabular}
\end{center}}\end{minipage}
}
\\
\centering
\vspace{0.5em}
%#################################################
% Type of Correlation Matrix in CA
%#################################################
\subfloat[
Calculation method for the correlation matrices in CA.
\label{tab:CalculationMethodInCA}
]{
\begin{minipage}{0.45\linewidth}{\begin{center}
% \tablestyle{4pt}{1.05}
\begin{tabular}{x{55}|x{25}}
\toprule[1pt]
Method & Avg. \\
\midrule
Addition & 65.9 \\
Subtraction & 65.8 \\
\rowcolor{gray!30}
Hadamard & \textbf{66.2} \\
\bottomrule[1pt]
\multicolumn{2}{c}{~}\\

\end{tabular}
\end{center}}\end{minipage}
}
\hspace{1.5em}
%#################################################
\subfloat[
Left and right boundaries $B_L$ and $B_R$ of $\gamma$ in MDWA-Loss.
\label{tab:GammaBoundaries}
]{
\begin{minipage}{0.45\linewidth}{\begin{center}
% \tablestyle{4pt}{1.05}
\begin{tabular}{x{67}|x{15}}
\toprule[1pt]
Boundaries of $\gamma$ & Avg. \\
\midrule
$B_L = B_R = 1$ & 65.1 \\
$B_L = 1, B_R = 1.5$ & 65.1 \\
\rowcolor{gray!30}
$B_L = 1, B_R = 2$ & \textbf{65.6} \\
$B_L = 1.5, B_R = 2$ & 65.2 \\
\bottomrule[1pt]
\end{tabular}
\end{center}}\end{minipage}
}

\end{table}
%##################################################################################################

==> Fig_Tab/Mislabel.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/Mislabel.pdf}
    \caption{
    Examples of mislabeled samples in BP4D (top) and DISFA (bottom). The annotations in the blue boxes and the red boxes represent the original annotations of the datasets and missed annotations, respectively.
    }
    \label{fig:mislabel}
\end{figure}

==> Fig_Tab/TSNE.tex <==
\begin{figure}
  \begin{minipage}{0.235\textwidth}
    \centering
    \includegraphics[width=0.75\linewidth]{figs/TsneNolossFigsize.png}
    \subcaption{w/o $\mathcal{L}_\text{MDWA}^{\prime}$}
    \label{fig:withoutLMoKE}
  \end{minipage}%
  \begin{minipage}{0.235\textwidth}
    \centering
    \includegraphics[width=0.75\linewidth]{figs/TsneFigsize.png}
    \subcaption{w/ $\mathcal{L}_\text{MDWA}^{\prime}$}
    \label{fig:withLMoKE}
  \end{minipage}
  \vspace{-0.7em}
  \caption{The t-SNE distribution of the [CLS] tokens from the final group of MoKEs.}
\label{fig:tsne}
\vspace{-0.8em}
\end{figure}

==> Fig_Tab/TuneLastLayer.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/TuneViTLayer.png}
    \caption{
    Average F1-score results on BP4D and the corresponding number of learnable parameters obtained by the partially fine-tuning paradigm.
    }
    \label{fig:TuneLastLayer}
\end{figure}
